Global explainability of a deep abstaining classifier

We present a global explainability method to characterize sources of errors in the histology prediction task of our real-world multitask convolutional neural network (MTCNN)-based deep abstaining classifier (DAC), for automated annotation of cancer pathology reports from NCI-SEER registries. Our classifier was trained and evaluated on 1.04 million hand-annotated samples and makes simultaneous predictions of cancer site, subsite, histology, laterality, and behavior for each report. The DAC framework enables the model to abstain on ambiguous reports and/or confusing classes to achieve a target accuracy on the retained (non-abstained) samples, but at the cost of decreased coverage. Requiring 97% accuracy on the histology task caused our model to retain only 22% of all samples, mostly the less ambiguous and common classes. Local explainability with the GradInp technique provided a computationally efficient way of obtaining contextual reasoning for thousands of individual predictions. Our method, involving dimensionality reduction of approximately 13000 aggregated local explanations, enabled global identification of sources of errors as hierarchical complexity among classes, label noise, insufficient information, and conflicting evidence. This suggests several strategies such as exclusion criteria, focused annotation, and reduced penalties for errors involving hierarchically related classes to iteratively improve our DAC in this complex real-world implementation.

==> abstract_prev.tex <==
% \abstract{
% We %developed a workflow to 
% analyzed a complex real-world \ac{CNN} based abstaining classifier of cancer pathology reports, trained on about 1.5 million free-text %electronic health records (EHRs) or 
% \ac{ePath} reports, received from   six cancer registries, describing results of the examination of malignant specimens to understand the determinants of classification and abstention.%, to generate a population-based information on new cancer diagnoses.
% \\
% \textbf{Background} %if any
% Previous work has shown that deep learning solutions based on \acp{CNN} can outperform rule-based classification methods when the focus is on robustness and generalizability.  In applications where  extremely low error rates are required, \acp{DAC} provide a generally-applicable solution, where the model is trained to not answer unless it can statistically guarantee high accuracy.  Abstention can, however, result in a significant decrease in sensitivity. Analysis of the determinants of classification and abstention can provide insight into how to iteratively improve the sensitivity and accuracy of the workflow. \\
% \textbf{Methods} %if any
% We computed \ac{LIME} and explanations based on saliency maps for the histology classification task for 10,000 lung and breast cancers \ac{ePath} reports, using our previously described \ac{DAC} tuned to an accuracy rate of 97\%.  We then carry out a \ac{PCA} and identify several strategies to subgroup reports according to likely determinants of classification errors and abstinence.\\
% \textbf{Results} %if any
% We show that saliency maps provide explanations that are qualitatively similar to \ac{LIME}, but using more than one hundred times less computer time.  We observe that the first two principal components of the explanation matrix enable distinct subgroups of reports to be identified.  For nonabstained reports, the well separated groups correspond to the common histology classes.  Essentially, all of the misclassification errors appeared to be due to inscrutable training or test labels, possibly reflecting label noise in such real-world  data.  For abstained reports, studying the histology category with the highest nonabstaining softmax score, results in a far richer grouping of reports.  \\
% \textbf{Conclusion} %if any
% By characterizing regions of \ac{PCA}-space according to classification/ misclassification type, keyword usage, and proclivity to abstain, we were able to identify regions of the PC1 vs PC2 plot containing reports associated with clear information, those with conflicting information, those with no information, and those classified using indirect information.  This provides insight into how to iteratively improve the overall sensitivity and accuracy of our workflow.
% }

\abstract{
\textbf{Objective}
Develop an end-to-end automated multitask text classifier for cancer pathology reports such that the model abstains (i.e., not answer) unless it can statistically guarantee high accuracy, and provides 
% human interpretable 
global explanations for classifications/abstentions.
\\
\textbf{Materials and Methods}
Previous work has shown a \acs{DAC} framework on an \acs{MTCNN} classifier with \acs{LIME} explainability to classify cancer pathology reports and provide local explanations for five tasks of interest to \acs{NCI}-\acs{SEER} registries 
% : cancer site, histology, subsite, laterality, and behavior.
such that each task is separately optimized.
We extend this work by introducing \textit{ntask} loss function that co-optimize multiple tasks.
% We introduced a modified abstention-based cross-entropy loss function to account for the abstention rates and accuracy across all tasks of interest such that the \textit{ntask} parameter is also tuned during model training. 
% To further enhance the trustworthiness and utility of the model in real world, 
We introduce a new approach to get global explainability of the model by applying PCA on saliency maps based local explanations for \acs{NLP}. 
% Particularly, we extensively study global explainability for histology to explore ways to reduce abstention.
% We project compute local explanations based on saliency maps for the histology classification task of cancer \ac{ePath} reports for the most common cancer sites.  
% Applying \ac{PCA} on the saliency maps based local explanations, we identify and visualize several regions/groups highlighting of global reasons for classification - correct predictions, errors, and abstinence.
\\
\textbf{Results} %if any
The \textit{ntask} loss function enables optimization of abstention vs accuracy across multiple tasks simultaneously and guarantees the desired accuracy across all tasks of interest, 
% enabling the desired level of accuracy on all tasks of interest, 
although with higher abstention. 
Visualization of the first two principal components applied on local explanations enables identification of several patterns of learning. 
%in the model.
For non-abstained reports in histology classification task, the well separated groups correspond to the common classes.  Essentially, all of the misclassifications appeared to be due to inscrutable training or test labels, possibly reflecting label noise in such real-world data.  For abstained reports, studying the histology category with the highest non-abstaining softmax score, results in a far richer grouping of reports.  
\\
\textbf{Discussion and Conclusion} %ifany
We demonstrate the utility of our \textit{ntask} classifier/loss function, combined with our global explainability.
% of characterizing regions of \acs{PCA}-space
Systematic analysis of such global explanations 
% obtained for predictions and abstention 
can facilitate quantifying practical value and potential risk of the model in real world as well as ways provide insights to iteratively improve the sensitivity of such workflows. 
%By characterizing regions of \ac{PCA}-space according to classification/ misclassification type, keyword usage, and proclivity to abstain, we were able to identify regions of the PC1 vs PC2 plot containing reports associated with clear information, those with conflicting information, those with no information, and those classified using indirect information.  This provides insight into how to iteratively improve the overall sensitivity and accuracy of our workflow.
}

==> figs/abs_acc.tex <==
\begin{figure}[ht]
        \centering
        \begin{tikzpicture}
            \begin{axis}[width=.85\textwidth,height=4in,
                    %legend style={at={(0.02,1.12)},anchor=north west},
                    xmin=0.75, xmax=1.0,
                    ymin=0.0, ymax=1.0,
                    legend pos=north west,
                    legend columns=1,
                    ylabel near ticks,
                    ylabel={\Large \textbf{Abstention}},
                    xlabel={\Large \textbf{Target Accuracy}},
                    xtick={0.75, 0.8, 0.85, 0.90, 0.95, 1.0},
                    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
                    yticklabel style = {font=\large, xshift=0.5ex},
                    xticklabel style = {font=\large, yshift=0.5ex},
                    ymajorgrids=true,
                    max space between ticks=20,
                    grid style=dashed,
                    legend style={nodes={scale=2}},
                    legend entries={ 
                    \textcolor{blue}{site}, \textcolor{black}{subsite}, \textcolor{green}{laterality}, \textcolor{red}{histology}, \textcolor{cyan}{behavior}, ntask
                    }]
            \addplot[blue,mark=*,line width=1.5] table {figs/abs_acc_data/site.tex};
            \addplot[black,mark=*, line width=1.5] table {figs/abs_acc_data/subsite.tex};
            \addplot[green,mark=*, line width=1.5] table {figs/abs_acc_data/laterality.tex};
            \addplot[red,mark=*, line width=1.5] table {figs/abs_acc_data/histology.tex};
            \addplot[cyan,mark=*, line width=1.5] table {figs/abs_acc_data/behavior.tex};
            % \addplot[cyan,mark=*, line width=1.0] table {figs/abs_acc_data/ntask.tex};
            \end{axis}
        \end{tikzpicture}
        %\includegraphics[width=1.0\linewidth]{BML_Intel_Offload.png}
        \caption{Plots of abstention vs accuracy for the multi-task classification problem,
        % including the Ntask parameter, 
        as accuracy target is varied from 80\% to 97\%.}
        \label{fig:abs_acc}
\end{figure}


==> figs/abs_acc_data/behavior.tex <==
0.9775  0.00
0.9771  0.00
0.9774  0.00
0.9776  0.00
0.9771  0.00
0.9788  0.00391
0.97874 0.00292

==> figs/abs_acc_data/histology.tex <==
0.8002  0.0531
0.8244  0.1189
0.8514  0.2045
0.8806  0.2976
0.9003  0.3726
0.9288  0.4795
0.9489  0.5996
0.97452 0.78445

==> figs/abs_acc_data/laterality.tex <==
0.9107  0.00
0.9109  0.00
0.9101  0.00
0.9109  0.00
0.9110  0.00
0.9285  0.0344
0.9495  0.0922
0.97586 0.21461

==> figs/abs_acc_data/ntask.tex <==
0.7984  0.335
0.8236  0.4019
0.8571  0.5073
0.8806  0.5755
0.8999  0.6284
0.9302  0.7027
0.9477  0.7685
0.97468 0.87323

==> figs/abs_acc_data/site.tex <==
0.9137  0.0
0.9132  0.00
0.9124  0.00
0.9122  0.00
0.9132  0.00
0.9305  0.0287
0.9523  0.0857
0.97596 0.17537

==> figs/abs_acc_data/subsite.tex <==
0.7991  0.3214
0.8291  0.3910
0.8593  0.4570
0.8815  0.4947
0.9043  0.5378
0.9315  0.5961
0.9523  0.6455
0.97478 0.72028


==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> methods/ntask.tex <==
\subsection*{N-task abstention} 

The original multi-task DAC requires individual tuning for each task to achieve the desired accuracy, with varying levels of abstention. The combined accuracy across multiple tasks is, as expected, slightly lower than the accuracy on each task, so to achieve a desired accuracy on multi-task classification, the target accuracy on each task needed to be increased to compensate for this loss. The degree to which each individual target accuracy must be increased is dependent on the abstention-accuracy curve for that task, as well as the correlation of abstention between tasks \cref{fig:mt_abs_acc}. 
This results in a multi-level tuning problem, where each user has to find a set of targets that achieves the desired multi-task accuracy, and reduces the coverage on each individual task. Additionally, it was decided by NCI that there was a benefit to improving the coverage on the individual tasks, even if not all 4 tasks of interest were classified for a single sample. This leads to the combined goal of finding the samples where all 4 tasks can be predicted with the required accuracy, as will as maximizing the fraction of non-abstained reports for each individual task, again at the required accuracy. Conceptually, this could be accomplished by training two separate models: one tuned to predict all 4 tasks with the desired accuracy (and the complexity of tuning mentioned above) and a second tuned to predict each individual task at the desired accuracy. The N-task method is an attempt to combine both these features into a single model and avoid the tuning issue described earlier.

% \input{figs/abs_acc}

[EXPAND]

We introduce the notion of a separate dummy task, with no existing ground truth, to attempt to identify those samples which we expect to be predicted with the desired accuracy on all the ’tasks of interest’ in the multi-task problem. To simplify the derivation, we consider the case where all the original tasks are tasks of interest. In the case where there
are additional tasks which are not ’of interest’ then they will simply use the original DAC loss function given by eq.(1).

To this end, we introduced a dummy task with binary outputs and no truth value, which indicated whether the sample should be abstained on whether or not the individual tasks decide to abstain. To minimize the dependence of the various optimizations (the abstention parameters $\alpha_i$ that controls the balance between coverage and abstention of each task and the abstention parameter $\alpha$ that controls the balance between n-task abstention and coverage), we decided to build the loss function of the dummy task out of the same cross-entropies that contribute to the loss function of each individual task shown in eq.(1).

To be precise, since the individual losses can be written as,
$\mathcal{L}_i = q_iS_i-\alpha_i \log q_i$ (where we have used the notation $q_i = 1 - p_{i,n_{i+1}}$ and $S_i = -\sum_{i}^{n_i} t_{ij} \log(p_{ij}/q_i))$, we defined the loss
for the dummy as 
$\mathcal{L}_d = q(PSi) - \alpha \log q.$
Summing all these pieces, one obtains:
\begin{equation}
    \mathcal{L}(x) = -\sum_{i}[(q_i + q)S_i - \alpha_i\log q_i] - \alpha \log q
\end{equation} 

This is not the only possible choice for the extra task: the expediency of building its loss out of the individual cross-entropies may not even be the best strategy. For example, one can build the dummy task by collapsing the multitask array into a prohibitively large single task with the number of classes given by the product of the number of classes in each task. We have not tried this and other similar approaches.

\subsection{Tuning the multi-task DAC for combined performance}
[EXPAND]

==> results/abs_acc.tex <==
\subsection*{Accuracy-abstention trade-off in \ac{DAC}}
% To the right side of Figure \ref{fig:model_arch} is shown the accuracy vs sensitivity trade-off as the \ac{DAC} is optimized for eight levels of accuracy, ranging from 80\% to 97\%.   Tuning our \ac{DAC} to 97\% greatly decreased the model sensitivity, to the extent that many minority classes were entirely eliminated.  The behavior task (in-situ, malignant, invasive, and metastatic) with 97\% accurate without an abstention category, while laterality and site suffered a modest decrease in sensitivity, to 82-84\% with the 97\% accuracy requirement.  Both subsite and histology tasks, however, lost most of their sensitivity when tuned for 97\% accuracy, with answers for just over 20\% of the reports.  This loss of sensitivity is not uniform across categories, however.  The histology of more than 94\% of prostate cancers, for example, is adenocarcinoma (code 8140), while lung and breast cancers have 2-3 dominant classes with a number of rare classes and the abstention rates are very different across site-histology combinations.

\cref{fig:abs_acc} shows the abstention (fraction of abstained reports) vs accuracy trade-off for all our classification tasks as the \ac{DAC} is optimized for eight levels of target accuracy, ranging from 80\% to 97\%.
Tuning our \ac{DAC} for 97\% accuracy resulted in a very high abstention, to the extent that many minority classes were entirely eliminated.  The behavior task (in-situ, malignant, invasive, and metastatic) was able to achieve 97\% accuraty with no abstention at all, while laterality and site suffered modest abstention, to 17.5-21.5\% with the 97\% accuracy requirement.  Both subsite and histology tasks, however, show exponential trends as the target accuracy is increased losing most of their coverage when tuned for 97\% accuracy, with answers for just over 20\% of the reports i.e. $\sim$ 80\% abstention.  This abstention is not uniform across tasks as well as across classes (or categories) within a task.  The histology of more than 94\% of prostate cancers, for example, is adenocarcinoma (code 8140), while lung and breast cancers have 2-3 dominant classes with a number of rare classes and the abstention rates are very different across site-histology combinations.

\input{figs/abs_acc}

% \begin{figure*}[htbp]
% 	\centering
%         \includegraphics[width=0.75\columnwidth]{figs/multitask_abs_acc.png}
% 	\hspace{0.1in}
% 	\caption{Plots of abstention versus accuracy for individual tasks in the multi-task classification problem. The 'behavior' task always exceeds the desired $97\%$ accuracy and is not shown. Tuning a multi-task classifier to achieve the desired accuracy on multiple tasks simultaneously requires heuristically tuning each task to a higher accuracy, such that the combined performance satisfies the desired accuracy. The degree of over-tuning for each task depends not only on the steepness of the individual abstention-accuracy for that task, but also the degree of correlation between that task and the other tasks to be included in the combined accuracy.}
% 	\label{fig:mt_abs_acc}
% \end{figure*}


==> results/confusion_matrices.tex <==
\subsection*{Patterns of learning with detailed analysis of confusion matrices}
Our approach towards global explainability 
% for the model with 97\% accuracy 
starts with the identification of major patterns of learning and confusion through logical analysis of the confusion matrices. Identifying such patterns can be tricky given that our model is answering several questions (tasks) simultaneously, each with a handful to several hundreds of classes, and complex hierarchical relationships between the classes across the different tasks. We focus our analyses on the larger (more common) classes considering our overall goal of minimizing human effort spent on manual annotation. Since histology is hierarchical based on cancer site, we pick two largest cancer site classes - breast and lung cancers, including 265,377 breast cancer reports and 137,578 lung cancer reports, accounting for $\sim$ 39\% of all reports. In addition, to make our confusion matrix analysis tractable we again restrict the confusion matrices to the 20 most common histology classes for each of breast and lung cancers respectively, accounting for 263,991 (99\%) breast cancer reports and 133,497 (97\%) lung cancer reports.

\begin{figure}[htbp]
	\centering
%	\begin{minipage}{width=0.5\textwidth}
	\includegraphics[width=0.49\textwidth]{mtcnn_C34histology_cm}
 	\includegraphics[width=0.49\textwidth]{mtcnn_C34abs_histology_cm}
%	\caption{ Confusion matrices for (left) non-abstained and (right) abstained histologies for correctly identified lung cancers}
%	\label{fig:Lungconfusion}
%	\end{minipage}
%\end{figure}
%
%\begin{figure}[htbp]
%	\centering
%	\begin{minipage}{width=0.5\textwidth}
	\includegraphics[width=0.49\textwidth]{mtcnn_C50histology_cm}
 	\includegraphics[width=0.49\textwidth]{mtcnn_C50abs_histology_cm}
%	\caption{Confusion matrices for (left) non-abstained and (right) abstained histologies for correctly identified breast cancers }
%	\label{fig:breastConfusion}
% \end{minipage}
        \caption{Confusion matrices for non-abstained (left) and second-choice in abstained (right) histology predictions for reports where the primary site was correctly identified as lung (top) and breast (bottom) cancer. \edit{Check that we only cut on primary site and not on secondary site being consistent with primary site.} The cells are color coded according to the counts in them on a logarithmic scale: blacks and darker blues indicating higher counts. Note that since the abstaining classifier attempts to get a high micro-precision (i.e., overall accuracy), most low-prevalence labels do not occur as predictions (columns) among the nonabstained cases, and high precision is reached for each of the classes predicted at a high freuqency.}
        \label{fig:confusion_matrix}
\end{figure}

\cref{fig:confusion_matrix} shows the confusion matrices, color-coded based on the $\log$ of the number of reports in the cells, for the top 20 histology classes for lung (top) and breast (bottom) cancer reports, with the classwise precision (PPV) and recall at the bottom and right respectively. The left panels show the confusion matrix for the winning softmax, including for abstention classes, while the right panels show the confusion matrix for the second highest softmax of the reports abstained in the left i.e. the model's potential predictions in the absence of abstention. The left panels clearly show that the model is abstaining on majority of the reports and only able to predict the most common classes with the high accuracy of 97\% - adenocarcinomas (\textit{8140}), squamous cell carcinomas (\textit{8070}), small cell carcinomas (\textit{8041}) and neuroendocrine carcinomas (\textit{8240}) for lung cancer reports, and ductal carcinomas (\textit{8500}) and lobular carcinomas (\textit{8520}) for breast cancer reports. While a first glance on the left panels might suggest that the model isn't learning beyond the common classes with the largest number of samples, the confusion matrices for the abstained reports based on the second highest softmax (right panels) suggest that the model is learning patterns of other classes. In fact, in comparison to Fig. \ref{fig:confusion_baseline} which is the histology confusion matrix for 20 most common classes for a non-abstaining baseline classifier, the learning pattern appears to be very similar, suggesting that the model cannot effectively maintain $\geq 97\%$ accuracy for rarer classes with fewer samples. 
As expected, Fig. \ref{fig:confusion_baseline} and the right panels of \cref{fig:confusion_matrix} show that while the confusion patterns in confusion are widely distributed across the top 20 classes, the top four largest histology classes for the given site dominate the confusion patterns. 


%% In \cref{fig:breast_cancer_consistency1}, we see that the pickups from \ac{LIME}~\cite{ribeiro2016should} and saliency maps~\cite{simonyan2013deep} are very correlated. A bunch of words with unclear relevance (without context) is picked up by saliency maps, but not by \ac{LIME}; there is almost nothing which is picked up by \ac{LIME} but not by saliency maps.  

%% In \cref{fig:breast_cancer_consistency2}, we see that this phenomenon persists if we take the sign into account.  As seen comparing \cref{fig:lung_cancer_consistency1,fig:lung_cancer_consistency2} and, especially, \cref{fig:prostate_cancer_consistency1,fig:prostate_cancer_consistency2}, these trends are, in fact, clearer in the signed comparisons than in the unsigned ones.

%% In addition, we notice only in the signed comparisons (i.e., in \cref{fig:breast_cancer_consistency2,fig:lung_cancer_consistency2,fig:prostate_cancer_consistency2}, but not in \cref{fig:breast_cancer_consistency1,fig:lung_cancer_consistency1,fig:prostate_cancer_consistency1}) that in the reports that were abstained on, the pickups were all at the lower end (except recordbreaktoken).  The negative and the positive sides look remarkably similar (are they exactly the same?)

%% (I am not clear about how the figure was generated: is there any meaning to the upper left and lower right quadrants?)
